A nonparametric algorithm for optimal stopping based on robust optimization

Optimal stopping is a fundamental class of stochastic dynamic optimization problems with numerous applications in finance and operations management. We introduce a new approach for solving computationally-demanding stochastic optimal stopping problems with known probability distributions. The approach uses simulation to construct a robust optimization problem that approximates the stochastic optimal stopping problem to any arbitrary accuracy; we then solve the robust optimization problem to obtain near-optimal Markovian stopping rules for the stochastic optimal stopping problem. In this paper, we focus on designing algorithms for solving the robust optimization problems that approximate the stochastic optimal stopping problems. These robust optimization problems are challenging to solve because they require optimizing over the infinite-dimensional space of all Markovian stopping rules. We overcome this challenge by characterizing the structure of optimal Markovian stopping rules for the robust optimization problems. In particular, we show that optimal Markovian stopping rules for the robust optimization problems have a structure that is surprisingly simple and finite-dimensional. We leverage this structure to develop an exact reformulation of the robust optimization problem as a zero-one bilinear program over totally unimodular constraints. We show that the bilinear program can be solved in polynomial time in special cases, establish computational complexity results for general cases, and develop polynomial-time heuristics by relating the bilinear program to the maximal closure problem from graph theory. Numerical experiments demonstrate that our algorithms for solving the robust optimization problems are practical and can outperform state-of-the-art simulation-based algorithms in the context of widely-studied stochastic optimal stopping problems from high-dimensional option pricing.

==> figures/simple_example.tex <==
\usetikzlibrary{arrows,backgrounds,snakes}

\begin{tikzpicture}
\begin{axis}[
	x tick label style={
		/pgf/number format/1000 sep=},
	ylabel=Population,
	enlargelimits=0.15,
	legend style={at={(0.5,-0.15)},
		anchor=north,legend columns=-1},
	ybar=5pt,% configures `bar shift'
	bar width=9pt,
	nodes near coords,
	point meta=y *10^-7 % the displayed number
]
\addplot 
	coordinates {(1930,50e6) (1940,33e6)
		 (1950,40e6) (1960,50e6) (1970,70e6)};

\addplot 
	coordinates {(1930,38e6) (1940,42e6) 
		(1950,43e6) (1960,45e6) (1970,65e6)};

\legend{Far,Near}
\end{axis}
\end{tikzpicture}


\begin{tikzpicture}[thick, framed]
    \filldraw[fill=green!20] (2,0) rectangle (5,1);% draw the box
    \draw (3,0) -- (3,1) node[above]{$\textsc{M}$};% draw the median
    \draw (5,0.5) -- (7,0.5);% draw right whisker
    \draw (2,0.5) -- (1,0.5);% draw left whisker
    \draw (7,0.39) -- (7,0.61);% draw vertical tab
    \draw (1,0.39) -- (1,0.61);% draw vertical tab
    \node[below] at (2,0) {$\textsc{Q1}$};% label the hinge
    \node[below] at (5,0) {$\textsc{Q3}$};% label the hinge
    \filldraw[ball color=red!80,shading=ball] (4,0.5) circle
        (0.06cm) node[above]{$\bar{x}$};% the mean
    \draw[<->] (2.3, -0.3) -- (4.7, -0.3)
        node[pos=0.5,below]{$\textsc{IQR}$}; % mark the IQR fences
    \draw[<->] (2, -0.8) -- (0,-0.8)
        node[pos=0.5,below]{$\textsc{1.5*IQR}$}; % left inner fence
    \draw[<->] (2,-1.4) -- (-2, -1.4)
        node[pos=0.5,below]{$\textsc{3*IQR}$};% left outer fence
    \draw[<->] (5, -0.8) -- (8,-0.8)
        node[midway,below]{$\textsc{1.5*IQR}$}; % right inner fence
    \draw[<->] (5,-1.4) -- (10, -1.4)
        node[pos=0.5,below]{$\textsc{3*IQR}$};% right outer fence
    %
    \node[below] at (9,0.7) {$\textbf{*}$}; % mild outlier on the right
    \node[below] at (-2.4,0.7) {$o$}; % extreme outlier on the left
    % Title
    \draw (3,2) node[above,xshift=0.7cm]{$ \textsc{Box and Whisker
        Plot}$};%
    % Axis
    \draw (-3,-2) -- (11,-2);
    % Note that the snaked line is drawn to 11.1 to force
    % TikZ to draw the final tick.
    \draw[snake=ticks,segment length=3cm] (-3,-2) -- (11,-2);
\end{tikzpicture}

%
%\begin{tikzpicture}[thick, framed]
%    \filldraw[fill=green!20] (2,0) rectangle (5,1);% draw the box
%    \draw (3,0) -- (3,1) node[above]{$\textsc{M}$};% draw the median
%    \draw (5,0.5) -- (7,0.5);% draw right whisker
%    \draw (2,0.5) -- (1,0.5);% draw left whisker
%    \draw (7,0.39) -- (7,0.61);% draw vertical tab
%    \draw (1,0.39) -- (1,0.61);% draw vertical tab
%    \node[below] at (2,0) {$\textsc{Q1}$};% label the hinge
%    \node[below] at (5,0) {$\textsc{Q3}$};% label the hinge
%    \filldraw[ball color=red!80,shading=ball] (4,0.5) circle
%        (0.06cm) node[above]{$\bar{x}$};% the mean
%    \draw[<->] (2.3, -0.3) -- (4.7, -0.3)
%        node[pos=0.5,below]{$\textsc{IQR}$}; % mark the IQR fences
%    \draw[<->] (2, -0.8) -- (0,-0.8)
%        node[pos=0.5,below]{$\textsc{1.5*IQR}$}; % left inner fence
%    \draw[<->] (2,-1.4) -- (-2, -1.4)
%        node[pos=0.5,below]{$\textsc{3*IQR}$};% left outer fence
%    \draw[<->] (5, -0.8) -- (8,-0.8)
%        node[midway,below]{$\textsc{1.5*IQR}$}; % right inner fence
%    \draw[<->] (5,-1.4) -- (10, -1.4)
%        node[pos=0.5,below]{$\textsc{3*IQR}$};% right outer fence
%    %
%    \node[below] at (9,0.7) {$\textbf{*}$}; % mild outlier on the right
%    \node[below] at (-2.4,0.7) {$o$}; % extreme outlier on the left
%    % Title
%    \draw (3,2) node[above,xshift=0.7cm]{$ \textsc{Box and Whisker
%        Plot}$};%
%    % Axis
%    \draw (-3,-2) -- (11,-2);
%    % Note that the snaked line is drawn to 11.1 to force
%    % TikZ to draw the final tick.
%    \draw[snake=ticks,segment length=1cm] (-3,-2) -- (11.1,-2);
%\end{tikzpicture}

==> tables/table_asymmetric_old.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sun Nov 15 13:05:57 2020
\begin{tabular}{cclcccc}
  \hline
  &&& \multicolumn{3}{c}{Initial Price} & \\
 $d$ & Method & Basis functions  & $\bar{x}_a = 90$ & $\bar{x}_a = 100$ & $\bar{x}_a = 110$& Num. of Sample Paths \\
 \hline
  8 & RO &  & \textbf{57.71 (0.14)} & \textbf{67.20 (0.59)} & \textbf{69.38 (0.53)} & $2 \times 10^3$ \\ 
    8 & LS & one, pricesKO, KOind, payoff & 56.21 (0.09) & 65.46 (0.02) & 67.91 (0.24) & $10^5$ \\ 
    8 & LS & one, pricesKO, payoff & 56.32 (0.01) & 65.74 (0.02) & 67.80 (0.27) & $10^5$ \\ 
    8 & LS & payoff, KOind, pricesKO & 56.21 (0.09) & 65.46 (0.02) & 67.91 (0.24) & $10^5$ \\ 
    8 & LS & pricesKO, payoff & 56.30 (0.02) & 65.74 (0.01) & 67.79 (0.27) & $10^5$ \\ 
    8 & LS & one, prices, payoff & 55.20 (0.09) & 61.99 (0.25) & 59.60 (0.28) & $10^5$ \\ 
    8 & LS & one & 45.67 (0.11) & 52.77 (0.06) & 48.48 (0.11) & $10^5$ \\ 
    8 & LS & one, KOind, prices & 52.16 (0.30) & 61.91 (0.16) & 63.62 (0.30) & $10^5$ \\ 
    8 & LS & one, prices & 48.35 (0.14) & 52.97 (0.04) & 50.54 (0.07) & $10^5$ \\ 
    8 & LS & one, pricesKO & 51.44 (0.33) & 61.58 (0.10) & 62.77 (0.21) & $10^5$ \\ 
    8 & LS & maxprice, KOind, pricesKO & 52.43 (0.26) & 61.99 (0.23) & 63.83 (0.41) & $10^5$ \\ 
    8 & Tree &  & 55.43 (0.11) & 62.95 (0.05) & 63.39 (0.37) & $10^5$ \\ 
   \hline
 16 & RO &  & \textbf{72.38 (0.17)} & \textbf{77.78 (0.30)} & 69.86 (0.87) & $2 \times 10^3$ \\ 
   16 & LS & one, pricesKO, KOind, payoff & 70.95 (0.56) & 75.61 (0.46) & \textbf{70.60 (0.06)} & $10^5$ \\ 
   16 & LS & one, pricesKO, payoff & 70.97 (0.60) & 75.71 (0.44) & 69.99 (0.09) & $10^5$ \\ 
   16 & LS & payoff, KOind, pricesKO & 70.95 (0.56) & 75.61 (0.46) & \textbf{70.60 (0.06)} & $10^5$ \\ 
   16 & LS & pricesKO, payoff & 70.98 (0.59) & 75.73 (0.44) & 69.99 (0.12) & $10^5$ \\ 
   16 & LS & one, prices, payoff & 67.82 (0.33) & 66.95 (0.56) & 56.31 (0.38) & $10^5$ \\ 
   16 & LS & one & 59.23 (0.13) & 56.34 (0.18) & 45.56 (0.03) & $10^5$ \\ 
   16 & LS & one, KOind, prices & 66.91 (0.14) & 70.92 (0.24) & 63.57 (0.20) & $10^5$ \\ 
   16 & LS & one, prices & 59.48 (0.03) & 57.69 (0.18) & 49.67 (0.11) & $10^5$ \\ 
   16 & LS & one, pricesKO & 66.74 (0.31) & 70.66 (0.12) & 62.29 (0.20) & $10^5$ \\ 
   16 & LS & maxprice, KOind, pricesKO & 67.19 (0.14) & 71.09 (0.28) & 63.99 (0.24) & $10^5$ \\ 
   16 & Tree &  & 69.08 (0.31) & 71.38 (0.55) & 55.09 (0.19) & $10^5$ \\ 
   \hline
 32 & RO &  & \textbf{84.57 (0.33)} & 79.16 (0.58) & 60.44 (0.52) & $2 \times 10^3$ \\ 
   32 & LS & one, pricesKO, KOind, payoff & 82.39 (0.14) & \textbf{79.18 (0.03)} & \textbf{62.95 (0.33)} & $10^5$ \\ 
   32 & LS & one, pricesKO, payoff & 82.44 (0.12) & 79.08 (0.26) & 62.28 (0.28) & $10^5$ \\ 
   32 & LS & payoff, KOind, pricesKO & 82.39 (0.14) & \textbf{79.18 (0.03)} & \textbf{62.95 (0.33)} & $10^5$ \\ 
   32 & LS & pricesKO, payoff & 82.44 (0.10) & 79.07 (0.26) & 62.27 (0.30) & $10^5$ \\ 
   32 & LS & one, prices, payoff & 73.77 (0.43) & 62.79 (0.16) & 48.78 (0.44) & $10^5$ \\ 
   32 & LS & one & 64.24 (0.07) & 50.67 (0.12) & 44.31 (0.09) & $10^5$ \\ 
   32 & LS & one, KOind, prices & 77.60 (0.35) & 71.11 (0.26) & 56.05 (0.50) & $10^5$ \\ 
   32 & LS & one, prices & 64.62 (0.01) & 55.14 (0.18) & 46.64 (0.01) & $10^5$ \\ 
   32 & LS & one, pricesKO & 77.43 (0.37) & 70.56 (0.37) & 55.24 (0.52) & $10^5$ \\ 
   32 & LS & maxprice, KOind, pricesKO & 77.76 (0.42) & 71.53 (0.19) & 56.27 (0.46) & $10^5$ \\ 
   32 & Tree &  & 77.48 (0.46) & 63.81 (0.31) & 51.03 (0.28) & $10^5$ \\ 
  \end{tabular}


==> tables/table_asymmetric_time.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Tue Jan  5 09:15:48 2021
\begin{tabular}{cclcccc}
  \hline
  &&& \multicolumn{3}{c}{Initial Price} & \\
 $d$ & Method & Basis functions  & $\bar{x}_a = 90$ & $\bar{x}_a = 100$ & $\bar{x}_a = 110$& Num. of Sample Paths \\
 \hline
  8 & RO &  & \textbf{25.61 ( 2.74)} & \textbf{21.47 ( 1.53)} & 26.04 ( 3.39) & $2 \times 10^3$ \\ 
    8 & LS & one, pricesKO, KOind, payoff &  3.29 ( 0.20) &  3.20 ( 0.31) &  3.24 ( 0.15) & $10^5$ \\ 
    8 & LS & one, pricesKO, payoff &  3.16 ( 0.20) &  3.05 ( 0.25) &  3.13 ( 0.21) & $10^5$ \\ 
    8 & LS & payoff, KOind, pricesKO &  3.76 ( 0.63) &  3.29 ( 0.58) &  3.05 ( 0.44) & $10^5$ \\ 
    8 & LS & pricesKO, payoff &  3.03 ( 0.14) &  2.89 ( 0.23) &  2.87 ( 0.12) & $10^5$ \\ 
    8 & LS & one, prices, payoff &  3.31 ( 0.56) &  2.97 ( 0.29) &  2.90 ( 0.24) & $10^5$ \\ 
    8 & LS & one &  0.89 ( 0.07) &  0.93 ( 0.06) &  0.94 ( 0.08) & $10^5$ \\ 
    8 & LS & one, KOind, prices &  3.39 ( 0.55) &  2.99 ( 0.26) &  2.98 ( 0.21) & $10^5$ \\ 
    8 & LS & one, prices &  2.63 ( 0.19) &  2.71 ( 0.22) &  2.72 ( 0.19) & $10^5$ \\ 
    8 & LS & one, pricesKO &  2.78 ( 0.35) &  2.62 ( 0.18) &  2.53 ( 0.21) & $10^5$ \\ 
    8 & LS & maxprice, KOind, pricesKO &  3.01 ( 0.13) &  2.85 ( 0.26) &  2.87 ( 0.08) & $10^5$ \\ 
    8 & Tree &  & 14.03 ( 1.18) & 18.99 ( 7.37) & \textbf{54.67 (10.40)} & $10^5$ \\ 
   \hline
 16 & RO &  & \textbf{18.12 ( 1.37)} & 19.34 ( 2.39) & \textbf{36.09 ( 4.41)} & $2 \times 10^3$ \\ 
   16 & LS & one, pricesKO, KOind, payoff &  5.55 ( 0.61) &  5.30 ( 0.34) &  5.01 ( 0.42) & $10^5$ \\ 
   16 & LS & one, pricesKO, payoff &  5.50 ( 0.78) &  5.23 ( 0.33) &  5.24 ( 0.33) & $10^5$ \\ 
   16 & LS & payoff, KOind, pricesKO &  4.74 ( 0.72) &  4.62 ( 0.54) &  4.55 ( 0.41) & $10^5$ \\ 
   16 & LS & pricesKO, payoff &  5.29 ( 0.37) &  5.18 ( 0.38) &  4.87 ( 0.26) & $10^5$ \\ 
   16 & LS & one, prices, payoff &  5.57 ( 0.55) &  4.93 ( 0.29) &  5.10 ( 0.32) & $10^5$ \\ 
   16 & LS & one &  1.17 ( 0.11) &  1.26 ( 0.08) &  1.24 ( 0.05) & $10^5$ \\ 
   16 & LS & one, KOind, prices &  6.21 ( 1.46) &  5.72 ( 0.76) &  5.16 ( 0.51) & $10^5$ \\ 
   16 & LS & one, prices &  6.02 ( 1.63) &  5.11 ( 1.25) &  4.86 ( 0.73) & $10^5$ \\ 
   16 & LS & one, pricesKO &  4.61 ( 0.62) &  4.58 ( 0.52) &  4.67 ( 0.58) & $10^5$ \\ 
   16 & LS & maxprice, KOind, pricesKO &  5.11 ( 0.64) &  4.90 ( 0.60) &  4.73 ( 0.27) & $10^5$ \\ 
   16 & Tree &  & 13.53 ( 0.73) & \textbf{46.26 ( 1.58)} &  8.44 ( 0.85) & $10^5$ \\ 
   \hline
 32 & RO &  & 16.87 ( 1.57) & 19.27 ( 1.61) & \textbf{31.07 ( 3.77)} & $2 \times 10^3$ \\ 
   32 & LS & one, pricesKO, KOind, payoff & 15.07 ( 2.97) & 11.55 ( 1.37) & 13.68 ( 2.69) & $10^5$ \\ 
   32 & LS & one, pricesKO, payoff & 15.29 ( 2.15) & 12.20 ( 1.68) & 13.04 ( 3.25) & $10^5$ \\ 
   32 & LS & payoff, KOind, pricesKO & 13.13 ( 2.59) & 10.96 ( 1.81) & 11.30 ( 1.81) & $10^5$ \\ 
   32 & LS & pricesKO, payoff & 15.11 ( 3.27) & 11.39 ( 1.91) & 11.62 ( 1.44) & $10^5$ \\ 
   32 & LS & one, prices, payoff & 16.78 ( 4.89) & 10.68 ( 1.52) & 11.92 ( 3.11) & $10^5$ \\ 
   32 & LS & one &  1.62 ( 0.60) &  1.51 ( 0.16) &  1.69 ( 0.74) & $10^5$ \\ 
   32 & LS & one, KOind, prices & 14.61 ( 2.44) & 10.77 ( 0.79) & 11.48 ( 1.94) & $10^5$ \\ 
   32 & LS & one, prices & 12.49 ( 3.23) & 10.42 ( 0.57) & 10.47 ( 0.84) & $10^5$ \\ 
   32 & LS & one, pricesKO & 13.61 ( 3.66) & 10.55 ( 0.43) & 11.02 ( 1.31) & $10^5$ \\ 
   32 & LS & maxprice, KOind, pricesKO & 12.63 ( 0.86) & 10.82 ( 1.36) & 11.60 ( 1.09) & $10^5$ \\ 
   32 & Tree &  & \textbf{29.49 (19.77)} & \textbf{29.37 (26.84)} & 10.74 ( 0.66) & $10^5$ \\ 
  \end{tabular}


==> tables/table_symmetric_old.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sun Nov 15 13:05:57 2020
\begin{tabular}{cclcccc}
  \hline
  &&& \multicolumn{3}{c}{Initial Price}& \\
 $d$ & Method & Basis functions & $\bar{x}_a = 90$ & $\bar{x}_a = 100$ & $\bar{x}_a = 110$ & Num. of Sample Paths \\
 \hline
  8 & RO &  & \textbf{54.69 (0.18)} & \textbf{67.89 (0.07)} & \textbf{75.69 (0.56)} & $2 \times 10^3$ \\ 
    8 & LS & one, pricesKO, KOind, payoff & 54.47 (0.53) & 67.26 (0.27) & 73.59 (0.32) & $10^5$ \\ 
    8 & LS & one, pricesKO, payoff & 54.52 (0.48) & 67.35 (0.33) & 73.87 (0.27) & $10^5$ \\ 
    8 & LS & payoff, KOind, pricesKO & 54.47 (0.53) & 67.26 (0.27) & 73.59 (0.32) & $10^5$ \\ 
    8 & LS & pricesKO, payoff & 54.60 (0.55) & 67.34 (0.33) & 73.87 (0.28) & $10^5$ \\ 
    8 & LS & one, prices, payoff & 54.53 (0.54) & 65.67 (0.29) & 68.20 (0.38) & $10^5$ \\ 
    8 & LS & one & 44.90 (0.13) & 57.13 (0.04) & 60.34 (0.06) & $10^5$ \\ 
    8 & LS & one, KOind, prices & 49.26 (0.21) & 63.05 (0.06) & 69.97 (0.24) & $10^5$ \\ 
    8 & LS & one, prices & 48.81 (0.25) & 60.02 (0.01) & 59.45 (0.11) & $10^5$ \\ 
    8 & LS & one, pricesKO & 48.91 (0.15) & 62.28 (0.08) & 69.82 (0.12) & $10^5$ \\ 
    8 & LS & maxprice, KOind, pricesKO & 51.04 (0.25) & 63.48 (0.13) & 70.09 (0.22) & $10^5$ \\ 
    8 & Tree &  & 54.55 (0.42) & 66.95 (0.36) & 71.24 (0.31) & $10^5$ \\ 
   \hline
 16 & RO &  & \textbf{71.35 (0.24)} & \textbf{83.07 (0.24)} & \textbf{82.70 (0.43)} & $2 \times 10^3$ \\ 
   16 & LS & one, pricesKO, KOind, payoff & 70.86 (0.43) & 80.99 (0.37) & 81.16 (0.47) & $10^5$ \\ 
   16 & LS & one, pricesKO, payoff & 70.90 (0.46) & 81.18 (0.33) & 80.82 (0.40) & $10^5$ \\ 
   16 & LS & payoff, KOind, pricesKO & 70.86 (0.43) & 80.99 (0.37) & 81.16 (0.47) & $10^5$ \\ 
   16 & LS & pricesKO, payoff & 70.84 (0.45) & 81.20 (0.33) & 80.80 (0.43) & $10^5$ \\ 
   16 & LS & one, prices, payoff & 70.19 (0.35) & 76.46 (0.19) & 69.48 (0.26) & $10^5$ \\ 
   16 & LS & one & 61.45 (0.09) & 70.22 (0.20) & 57.74 (0.22) & $10^5$ \\ 
   16 & LS & one, KOind, prices & 65.25 (0.13) & 77.16 (0.09) & 74.53 (0.58) & $10^5$ \\ 
   16 & LS & one, prices & 64.01 (0.13) & 70.29 (0.24) & 59.85 (0.09) & $10^5$ \\ 
   16 & LS & one, pricesKO & 64.63 (0.05) & 76.87 (0.02) & 74.15 (0.63) & $10^5$ \\ 
   16 & LS & maxprice, KOind, pricesKO & 66.46 (0.18) & 77.40 (0.03) & 74.59 (0.55) & $10^5$ \\ 
   16 & Tree &  & 70.66 (0.43) & 79.70 (0.13) & 74.38 (0.51) & $10^5$ \\ 
   \hline
 32 & RO &  & \textbf{86.23 (0.35)} & \textbf{93.07 (0.74)} & 78.98 (0.35) & $2 \times 10^3$ \\ 
   32 & LS & one, pricesKO, KOind, payoff & 85.01 (0.34) & 91.05 (0.28) & \textbf{79.76 (0.36)} & $10^5$ \\ 
   32 & LS & one, pricesKO, payoff & 85.06 (0.37) & 91.11 (0.37) & 78.51 (0.35) & $10^5$ \\ 
   32 & LS & payoff, KOind, pricesKO & 85.01 (0.34) & 91.05 (0.28) & \textbf{79.76 (0.36)} & $10^5$ \\ 
   32 & LS & pricesKO, payoff & 85.06 (0.38) & 91.12 (0.33) & 78.49 (0.36) & $10^5$ \\ 
   32 & LS & one, prices, payoff & 82.20 (0.18) & 81.24 (0.40) & 61.18 (0.27) & $10^5$ \\ 
   32 & LS & one & 76.13 (0.09) & 72.03 (0.31) & 52.24 (0.14) & $10^5$ \\ 
   32 & LS & one, KOind, prices & 80.42 (0.15) & 86.12 (0.20) & 68.39 (0.50) & $10^5$ \\ 
   32 & LS & one, prices & 77.20 (0.23) & 71.89 (0.14) & 54.53 (0.18) & $10^5$ \\ 
   32 & LS & one, pricesKO & 80.08 (0.14) & 86.12 (0.11) & 65.39 (0.95) & $10^5$ \\ 
   32 & LS & maxprice, KOind, pricesKO & 81.06 (0.13) & 86.25 (0.18) & 68.76 (0.62) & $10^5$ \\ 
   32 & Tree &  & 84.53 (0.28) & 86.42 (0.37) & 60.94 (0.43) & $10^5$ \\ 
  \end{tabular}


==> tables/table_symmetric_time.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Tue Jan  5 09:15:48 2021
\begin{tabular}{cclcccc}
  \hline
  &&& \multicolumn{3}{c}{Initial Price}& \\
 $d$ & Method & Basis functions & $\bar{x}_a = 90$ & $\bar{x}_a = 100$ & $\bar{x}_a = 110$ & Num. of Sample Paths \\
 \hline
  8 & RO &  & \textbf{33.48 ( 4.21)} & \textbf{28.61 ( 1.76)} & \textbf{31.71 ( 1.94)} & $2 \times 10^3$ \\ 
    8 & LS & one, pricesKO, KOind, payoff &  3.35 ( 0.21) &  3.53 ( 0.50) &  3.14 ( 0.22) & $10^5$ \\ 
    8 & LS & one, pricesKO, payoff &  3.24 ( 0.20) &  2.97 ( 0.29) &  2.94 ( 0.23) & $10^5$ \\ 
    8 & LS & payoff, KOind, pricesKO &  3.52 ( 0.83) &  2.97 ( 0.28) &  3.03 ( 0.44) & $10^5$ \\ 
    8 & LS & pricesKO, payoff &  3.04 ( 0.25) &  2.81 ( 0.22) &  2.84 ( 0.19) & $10^5$ \\ 
    8 & LS & one, prices, payoff &  3.08 ( 0.18) &  2.97 ( 0.25) &  2.99 ( 0.10) & $10^5$ \\ 
    8 & LS & one &  0.86 ( 0.07) &  0.88 ( 0.03) &  0.93 ( 0.05) & $10^5$ \\ 
    8 & LS & one, KOind, prices &  3.13 ( 0.29) &  2.99 ( 0.32) &  2.92 ( 0.28) & $10^5$ \\ 
    8 & LS & one, prices &  2.64 ( 0.19) &  2.63 ( 0.15) &  2.62 ( 0.13) & $10^5$ \\ 
    8 & LS & one, pricesKO &  2.72 ( 0.34) &  2.77 ( 0.17) &  2.57 ( 0.17) & $10^5$ \\ 
    8 & LS & maxprice, KOind, pricesKO &  3.02 ( 0.15) &  2.99 ( 0.32) &  2.87 ( 0.08) & $10^5$ \\ 
    8 & Tree &  & 14.56 ( 1.01) & 13.29 ( 0.74) & 14.66 ( 2.91) & $10^5$ \\ 
   \hline
 16 & RO &  & \textbf{27.91 ( 2.38)} & \textbf{26.53 ( 2.65)} & \textbf{32.80 ( 3.45)} & $2 \times 10^3$ \\ 
   16 & LS & one, pricesKO, KOind, payoff &  5.49 ( 0.62) &  5.15 ( 0.17) &  5.20 ( 0.24) & $10^5$ \\ 
   16 & LS & one, pricesKO, payoff &  5.29 ( 1.02) &  4.84 ( 0.43) &  5.10 ( 0.33) & $10^5$ \\ 
   16 & LS & payoff, KOind, pricesKO &  4.71 ( 0.44) &  4.64 ( 0.30) &  4.61 ( 0.32) & $10^5$ \\ 
   16 & LS & pricesKO, payoff &  5.17 ( 0.71) &  4.82 ( 0.15) &  4.74 ( 0.25) & $10^5$ \\ 
   16 & LS & one, prices, payoff &  4.86 ( 0.81) &  4.69 ( 0.41) &  4.97 ( 0.10) & $10^5$ \\ 
   16 & LS & one &  1.27 ( 0.15) &  1.21 ( 0.08) &  1.22 ( 0.08) & $10^5$ \\ 
   16 & LS & one, KOind, prices &  6.24 ( 1.34) &  5.69 ( 1.28) &  5.50 ( 0.69) & $10^5$ \\ 
   16 & LS & one, prices &  5.97 ( 1.17) &  5.51 ( 1.55) &  5.01 ( 0.87) & $10^5$ \\ 
   16 & LS & one, pricesKO &  4.30 ( 0.30) &  4.17 ( 0.29) &  4.45 ( 0.31) & $10^5$ \\ 
   16 & LS & maxprice, KOind, pricesKO &  5.12 ( 0.61) &  4.68 ( 0.27) &  4.63 ( 0.28) & $10^5$ \\ 
   16 & Tree &  & 14.35 ( 0.91) & 13.79 ( 1.22) & 23.16 ( 5.71) & $10^5$ \\ 
   \hline
 32 & RO &  & \textbf{25.83 ( 2.23)} & \textbf{25.33 ( 2.81)} & \textbf{54.47 ( 8.76)} & $2 \times 10^3$ \\ 
   32 & LS & one, pricesKO, KOind, payoff & 13.73 ( 1.39) & 13.32 ( 2.22) & 12.00 ( 1.35) & $10^5$ \\ 
   32 & LS & one, pricesKO, payoff & 15.42 ( 3.90) & 15.33 ( 2.99) & 12.89 ( 2.17) & $10^5$ \\ 
   32 & LS & payoff, KOind, pricesKO & 13.05 ( 3.69) & 11.33 ( 1.27) & 11.66 ( 2.39) & $10^5$ \\ 
   32 & LS & pricesKO, payoff & 14.63 ( 2.31) & 14.01 ( 3.91) & 11.35 ( 1.54) & $10^5$ \\ 
   32 & LS & one, prices, payoff & 15.18 ( 5.56) & 14.17 ( 3.53) & 11.73 ( 1.72) & $10^5$ \\ 
   32 & LS & one &  2.13 ( 1.23) &  1.78 ( 0.93) &  1.67 ( 0.73) & $10^5$ \\ 
   32 & LS & one, KOind, prices & 13.25 ( 2.33) & 12.38 ( 2.44) & 11.95 ( 1.75) & $10^5$ \\ 
   32 & LS & one, prices & 12.23 ( 2.71) & 10.83 ( 1.02) & 10.91 ( 0.80) & $10^5$ \\ 
   32 & LS & one, pricesKO & 14.55 ( 4.76) & 11.12 ( 1.10) & 10.56 ( 0.60) & $10^5$ \\ 
   32 & LS & maxprice, KOind, pricesKO & 12.05 ( 1.72) & 10.92 ( 0.83) & 10.93 ( 1.42) & $10^5$ \\ 
   32 & Tree &  & 17.43 ( 1.34) & 17.14 ( 1.96) & 11.46 ( 2.27) & $10^5$ \\ 
  \end{tabular}

